I Cast Detect Thoughts: Learning to Converse and Guide with Intents and Theory-of-Mind in Dungeons and Dragons

We propose a novel task, G4C, to study teacher-student natural language interactions in a goal-driven and grounded environment. Dungeons and Dragons (D&D), a role-playing game, provides an ideal setting to investigate such interactions. Here, the Dungeon Master (DM), i.e., the teacher, guides the actions of several players -- students, each with their own personas and abilities -- to achieve shared goals grounded in a fantasy world. Our approach is to decompose and model these interactions into (1) the DM's intent to guide players toward a given goal; (2) the DM's guidance utterance to the players expressing this intent; and (3) a theory-of-mind (ToM) model that anticipates the players' reaction to the guidance one turn into the future. We develop a novel reinforcement learning (RL) method for training a DM that generates guidance for players by rewarding utterances where the intent matches the ToM-anticipated player actions. Human and automated evaluations show that a DM trained to explicitly model intents and incorporate ToM of the players using RL generates better-quality guidance that is 3x more likely to fulfill the DM's intent than a vanilla natural language generation (NLG) approach.

==> sections/data__deprecated_.tex <==
% \pei{Key Takeaway: After casting dialogue generation as a sequential decision making problem and view the next-turn listener action/utterance as feedback (section 2), we apply IDM idea on text data to label guidance (speaker action) on raw corpora. Move details to appendix}
% 3.3 feels different than 3.1; 3.2



\subsection{Inverse Dynamics Models (IDM) to Label Guidance}\label{sec:3.2}
\pei{This subsection needs some help on how to frame IDM and explain clearly about forward/backward modeling}
To train models to generate guidance as DM, we need to 
\textbf{identify posts that contain guidance and extract \emph{``guiding sentence''}} (the key sentence that leads the player to perform certain actions). Details about how we process the raw data to find a non-chitchat thread-like dialogue between the DM and players are presented in Appendix~\ref{appendix: cleaning detail}. Here we propose our method that locates guidance in raw PBP data by training a labeler on a small amount of human-labeled data using Inverse Dynamics Models.
% Look at previous 20 turns
% Find DM turns with name mention of the player using the action tag: “name_mention: xxx” OR with a “reply_to” and that previous turn is from the player
% If no text has been added in 20 turns, add the closest turn from DM if it’s not only replying to another player [D]
% Add turns from the player or DM before the earliest DM Text turn to the context [C]



% lots of pieces, help readers understand
% double budget
\paragraph{Intuition}\label{sec:3.3-int}




% FOLLOWING FROM VPT PAPER for reference
% we propose generating pseudo-labels by
% gathering a small amount of labeled data to train an inverse dynamics model (IDM) that predicts
% the action taken at each timestep in a video. Behavioral cloning (BC) can require a large amount
% of data because the model must learn to infer intent and the distribution over future behaviors from
% only past observations. In contrast, the inverse dynamics modeling task is simpler because it is
% non-causal, meaning it can look at both past and future frames to infer actions. In most settings,
% environment mechanics are far simpler than the breadth of human behavior that can take place within
% the environment, suggesting that non-causal IDMs could require far less data to train than causal BC
% models. Using pseudo-labels generated from the IDM, we then train a model to mimic the distribution
% of behavior in the previously unlabeled dataset with standard behavioral cloning at scale, which does
% not require any model rollouts and thus does not suffer from any potential exploration bottlenecks
% in the environment

% \paragraph{}

% % \begin{enumerate}
% %     \item Interface (3 questions)
% %     \item Agreement and analysis
% % \end{enumerate}

% \subsection{Training IDM}
% \begin{enumerate}
%     \item Training details
%     \item Evaluation
% \end{enumerate}

% \vspace{12cm}
